An Empirical Study of AI-based Smart Contract Creation

The introduction of large language models (LLMs) like ChatGPT and Google Palm2 for smart contract generation seems to be the first well-established instance of an AI pair programmer. LLMs have access to a large number of open-source smart contracts, enabling them to utilize more extensive code in Solidity than other code generation tools. Although the initial and informal assessments of LLMs for smart contract generation are promising, a systematic evaluation is needed to explore the limits and benefits of these models. The main objective of this study is to assess the quality of generated code provided by LLMs for smart contracts. We also aim to evaluate the impact of the quality and variety of input parameters fed to LLMs. To achieve this aim, we created an experimental setup for evaluating the generated code in terms of validity, correctness, and efficiency. Our study finds crucial evidence of security bugs getting introduced in the generated smart contracts as well as the overall quality and correctness of the code getting impacted. However, we also identified the areas where it can be improved. The paper also proposes several potential research directions to improve the process, quality and safety of generated smart contract codes.

==> intro-draft.tex <==
In the recent years, generative pre-trained transformer (GPT) models, natural language generation technique powered by deep-learning, have advanced to a state that is ready for mainstream adoption. Among the many applications enabled by the GPT models is source code generation from natural human language. For instance, when provided with a programming task in English, GitHub Copilot based on GPT-3 Codex model is capable of generating solution code satisfying the natural language specification.  The Codex model is trained on a large scale dataset of source codes in a dozen programming languages. It can convert code comments and specification to compilable source code at entire function or class level. Another example is ChatGPT. ChatGPT is also built on top of the GPT-3 family of generative models. It has been fine tuned using  supervised learning and a process of reinforcement learning, called RLHF (reinforcement learning from human feedback). Both fine-tuning approaches were designed to use human trainer feedback to improve the model's performance. Like Copilot, ChatGPT is capable of generating source code from natural language input. 

Both language generative models and tools have attracted strong public interests including the research community. In particular, researchers have investigated and evaluated the capability of the GPT models for generating source code. For instance, in ~\cite{}, the authors assessed the security risk of software code generated by Copilot against the code weakness enumerations by MITRE. 

The existing work has mostly focused on security assessment of these generative models for code generation targeting some specific programming languages like Python. There is a need to broaden the study of the generative models for code generation to cover more diverse programming languages as well as assess the generated software from more comprehensive dimensions beyond security risk. 

To fill the gap, in this report, we have explored both Copilot and ChatGPT for generating solidity smart contract code. We compared the code generation process and the generated smart contracts using both tools. The generated code was systematically evaluated. The main contributions are:


# first explore and evaluate AI feasibility and quality for creating smart contract code
# compare chatgpt and coplit
# evaluate using multiple metrics

==> results.tex <==
size of contract

auction:  4.747KB
ai generated:  2.286KB

BlackScholesEstimate 2.399
BlackScholesEstimateAI       ·      2.371

+
gas fee example
 
                 AI 		       Manual	
	            min	   max	    min	max
bid	            2678	43075	0	66135
highestBid	    526	526	        0	816
highestBidder	486	486	        0	596
endPrice	    504	504	        0	658




